A Combination of Testability and Decodability by Tensor Products

Ben-Sasson and Sudan (RSA 2006) showed that repeated tensor products of linear codes with a very large distance are locally testable. Due to the requirement of a very large distance the associated tensor products could be applied only over sufficiently large fields. Then Meir (SICOMP 2009) used this result (as a black box) to present a combinatorial construction of locally testable codes that match best known parameters. As a consequence, this construction was obtained over sufficiently large fields. In this paper we improve the result of Ben-Sasson and Sudan and show that for \emph{any} linear codes the associated tensor products are locally testable. Consequently, the construction of Meir can be taken over any field, including the binary field. Moreover, a combination of our result with the result of Spielman (IEEE IT, 1996) implies a construction of linear codes (over any field) that combine the following properties: have constant rate and constant relative distance; have blocklength $n$ and testable with $n^{\epsilon}$ queries, for any constant $\epsilon > 0$; linear time encodable and linear-time decodable from a constant fraction of errors. Furthermore, a combination of our result with the result of Guruswami et al. (STOC 2009) implies a similar corollary regarding the list-decodable codes.

==> abbreviations.tex <==

\newcommand\xth{\textsuperscript{th}\xspace}
\newcommand\xrd{\textsuperscript{rd}\xspace}
\newcommand\xst{\textsuperscript{st}\xspace}
\newcommand\xnd{\textsuperscript{nd}\xspace}


%--------------------------------------------------


% write something if the first argument is non-empty
\newcommand{\fornonempty}[2]{\ifthenelse{\equal{#1}{}}{}{#2}}
\newcommand{\emptyornot}[3]{\ifthenelse{\equal{#1}{}}{#2}{#3}}

\newcommand{\mathify}[1]{\ifmmode{#1}\else\mbox{$#1$}\fi}
\newcommand{\inlineordisplay}[2]{\ifinner {#2} \else {#1} \fi}
\newcommand{\displayorinline}[2]{\ifinner {#1} \else {#2} \fi}


\newcommand{\forallf}[2]{\forall \, {#1} \; \Bigsbrace{#2}}
\newcommand{\existf}[2]{\exists \, {#1} \; \Bigsbrace{#2}}
\newcommand{\existsf}[2]{\exists \, {#1} \; \Bigsbrace{#2}}


% Complexity classes
%-----------------------------------------------------
\newcommand{\paramcomplexityclass}[2]{{\bf #1}\left(#2\right)\xspace}
\newcommand{\complexityclass}[1]{{\bf #1}\xspace}
\renewcommand{\P}{\complexityclass{P}}
\newcommand{\EXPTIME}{\complexityclass{EXPTIME}}
\newcommand{\NEXPTIME}{\complexityclass{NEXPTIME}}
\newcommand{\NP}{\complexityclass{NP}}
\newcommand{\NPC}{\complexityclass{NPC}}
\newcommand{\CONP}{\complexityclass{coNP}}
\newcommand{\CNP}{\complexityclass{coNP}}
\newcommand{\RP}{\complexityclass{RP}}
\newcommand{\CORP}{\complexityclass{coRP}}
\newcommand{\CRP}{\complexityclass{coRP}}
\newcommand{\DL}{\complexityclass{L}}
\newcommand{\NL}{\complexityclass{NL}}
\newcommand{\CONL}{\complexityclass{coNL}}
\newcommand{\CNL}{\complexityclass{coNL}}
\newcommand\SIGMATWO{\complexityclass{\Sigma_2}}
\newcommand\SIGMATHREE{\complexityclass{\Sigma_3}}
\newcommand\PITWO{\complexityclass{\Pi_2}}
\newcommand\PITHREE{\complexityclass{\Pi_3}}
\newcommand\PSPACE{\complexityclass{PSPACE}}
\newcommand\SHARPP{\complexityclass{\#P}}
\newcommand\PARITYP{\complexityclass{$\oplus$P}}
\newcommand\PH{\complexityclass{PH}}
\newcommand\PHEIRARCHY{\complexityclass{PH}}
\newcommand\IP{\complexityclass{IP}}
\newcommand\PCP{\complexityclass{PCP}}
\newcommand\PCPP{\complexityclass{PCPP}}
\newcommand\NTIME[1]{\paramcomplexityclass{NTIME}{#1}}
\newcommand\DTIME[1]{\paramcomplexityclass{DTIME}{#1}}
\newcommand\NSPACE[1]{\paramcomplexityclass{NSPACE}{#1}}
\newcommand\DSPACE[1]{\paramcomplexityclass{DSPACE}{#1}}
\newcommand\CNTIME[1]{\paramcomplexityclass{coNTIME}{#1}}
\newcommand\CNSPACE[1]{\paramcomplexityclass{coNSPACE}{#1}}
\newcommand\PPT{\complexityclass{PPT}}
\newcommand\MIP{\complexityclass{MIP}}

\newcommand\GENCLASS{\mbox{$\cal C$}\xspace}
\newcommand\COGENCLASS{\mbox{\bf co$\cal C$}\xspace}

%-----------------------------------------------------

% Specific Computational Problems/Languages
%-----------------------------------------------------
\newcommand\lang[1]{\mbox{\sc #1}\xspace}
%\newcommand\paramlang[2]{\mbox{\sc #1}\paren{\mathify{#2}}\xspace}
\newcommand\paramlang[2]{\mbox{\sc #1}\fornonempty{#2}{\paren{\mathify{#2}}}\xspace}
\newcommand\SAT{\lang{SAT}}
\newcommand\MAXTSAT[1][]{\mathify{\paramlang{MAX-3SAT}{#1}}}
\newcommand\MAXTLIN{\lang{MAX-3LIN}}
\newcommand\TQBF{\lang{TQBF}}
\newcommand\permp{\lang{PERMANENT}}
\def\perm{\operatorname{perm}} % <- E.R.: not sure what this does
%-----------------------------------------------------

% Sets of Interest
%-----------------------------------------------------
\newcommand\nat{\mathify{\mathbb{N}}}
\newcommand\ints{\mathify{\mathbb{Z}}}
\newcommand\posints{\mathify{\mathbb{N}^{+}}}
\newcommand\reals{\mathify{\mathbb{R}}}
\newcommand\posreals{\mathify{\mathbb{R}^{+}}}
\newcommand\rationals{\mathify{\mathbb{Q}}}
\newcommand\complexes{\mathify{\mathbb{C}}}
\newcommand{\zo}{\set{0,1}}
\newcommand{\pmo}{\set{1,-1}}
%-----------------------------------------------------

% functions

\newcommand{\fnrngdom}[2]{#1\!\!\rightarrow#2}
\newcommand{\fndef}[3]{{#1\,:\,\fnrngdom{#2}{#3}}}
\newcommand\poly[1]{\mathify{\mathop{\rm poly}\!\left(#1\right)}}
\newcommand\polylog[1]{\mathify{\mathop{\rm polylog}\!\left(#1\right)}}
\newcommand\loglog[1]{\mathify{\mathop{\rm log\,log}\!\left(#1\right)}}
\newcommand{\floor}[1]{\mathify{\left\lfloor\, #1\,\right\rfloor}}
\newcommand{\ceil}[1]{\mathify{\left\lceil\, #1\,\right\rceil}}
\newcommand{\eqdef}{{\quad{\stackrel{\rm def}{=}}\quad}}
\newcommand{\rest}[2]{{{#1}}\downharpoonleft_{{#2}}}


% arrows and relation symbols
\newcommand\xor{\oplus}
\newcommand\bxor{\bigoplus}

%% probability stuff

\newcommand{\pr}[2]{{\mathop{\mathbf{Pr}}_{#1}\!{\left[{#2}\right]}}}
\newcommand{\cpr}[3]{{\mathop{\mathbf{Pr}}_{#1}\!{\left[{#2} \middle| {#3} \right]}}}
\newcommand{\ex}[2]{{\mathop{\mathbf{E}}_{#1}\!{\left[{#2}\right]}}}
\newcommand{\cex}[3]{{\mathop{\mathbf{E}}_{#1}\!{\left[{#2} \middle| {#3} \right]}}}
\newcommand{\var}[2]{{\mathop{\mathbf{Var}}_{#1}\!{\left[{#2}\right]}}}
\newcommand{\covar}[2]{{\mathop{\mathbf{Cov}}_{#1}\!{\left[{#2}\right]}}}

% Parentheses, Braces, Norms etc.
%-------------------------------------------------------
\newcommand{\paren}[1]{{\left({#1}\right)}}
\newcommand{\angles}[1]{{\langle{#1}\rangle}}
\newcommand{\abs}[1]{\mathify{\left| #1 \right|}}
\newcommand{\size}[1]{\mathify{\left| #1 \right|}}
\newcommand{\set}[1]{\mathify{\left\{#1\right\}}}
\newcommand{\cond}[2]{{#1} \: \big| \: {#2}}
\newcommand{\condset}[2]{{\left\{ {#1} \: \middle| \: {#2} \right\}}}
\newcommand{\enum}[2]{{#1}_{1},\ldots, {#1}_{#2}}
\newcommand{\nset}[2]{\set{\enum{#1}{#2}}}
\newcommand{\npar}[2]{\paren{\enum{#1}{#2}}}
\newcommand{\inpr}[2]{\angles{{#1},{#2}}}


% Stacking
%-------------------------------------------------------
\newcommand{\ubstack}[2]{\mathop{\,\underbrace{#1}\,}_{#2}}
\newcommand{\obstack}[2]{\mathop{\overbrace{#1}}^{#2}}
%this stacks two lines, centered... it's ugly!
% use \begin{aligned)first \\ second \end{aligned} instead
\newcommand{\twolines}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}

% Shorthands
%-------------------------------------------------------
\newcommand {\acc}{\mbox{{\sf accept}}\xspace}
\newcommand {\rej}{\mbox{{\sf reject}}\xspace}
%-------------------------------------------------------

% Greek letters
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\w}{\omega}
\newcommand{\s}{\sigma}
\newcommand{\z}{\zeta}
\newcommand{\m}{\mu}

% Caligraphic letters

\newcommand{\A}{{\cal A}}
\newcommand{\B}{{\cal{B}}}
\newcommand{\C}{{\cal{C}}}
\newcommand{\D}{{\cal{D}}}
\newcommand{\E}{{\cal{E}}}
\newcommand{\F}{{\cal{F}}}
\newcommand{\G}{{\cal{G}}}
\renewcommand{\H}{{\cal{H}}}
\newcommand{\I}{{\cal{I}}}
\newcommand{\J}{{\cal{J}}}
\newcommand{\K}{{\cal{K}}}
\renewcommand{\L}{{\cal{L}}}
\newcommand{\cL}{{\cal{L}}}
\newcommand{\M}{{\cal{M}}}
\newcommand{\N}{{\cal{N}}}
\renewcommand{\O}{{\cal{O}}}
%\newcommand{\P}{{\cal{P}}}
\newcommand{\Q}{{\cal{Q}}}
\newcommand{\R}{{\cal{R}}}
\renewcommand{\S}{{\cal{S}}}
\newcommand{\T}{{\cal{T}}}
\newcommand{\U}{{\cal{U}}}
\newcommand{\V}{{\cal{V}}}
\newcommand{\W}{{\cal{W}}}
\newcommand{\X}{{\cal{X}}}
\newcommand{\Y}{{\cal{Y}}}
\newcommand{\Z}{{\cal{Z}}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical operators

\DeclareMathOperator{\krn}{ker}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\rnk}{rank}

\newcommand{\remove}[1]{}

